Magnetic-field resilience of 3D transmons with thin-film Al/AlO$_x$/Al Josephson junctions approaching 1 T

Magnetic-field-resilient superconducting circuits enable sensing applications and hybrid quantum-computing architectures involving spin or topological qubits and electro-mechanical elements, as well as studying flux noise and quasiparticle loss. We investigate the effect of in-plane magnetic fields up to 1 T on the spectrum and coherence times of thin-film 3D aluminum transmons. Using a copper cavity, unaffected by strong magnetic fields, we can solely probe the magnetic-field effect on the transmons. We present data on a single-junction and a SQUID transmon, that were cooled down in the same cavity. As expected, transmon frequencies decrease with increasing fields, due to a suppression of the superconducting gap and a geometric Fraunhofer-like contribution. Nevertheless, the thin-film transmons show strong magnetic-field resilience: both transmons display microsecond coherence up to at least 0.65 T, and $T_1$ remains above 1 $\mathrm{\mu}$s over the entire measurable range. SQUID spectroscopy is feasible up to 1 T, the limit of our magnet. We conclude that thin-film aluminum Josephson junctions are a suitable hardware for superconducting circuits in the high-magnetic-field regime.

==> Definitions.tex <==

% T1, T2 T2echo
\newcommand{\Tone}{T_{1}}
\newcommand{\Ttwo}{T_{2}}
\newcommand{\Ttwostar}{T_{2}^{\mathrm{*}}}
\newcommand{\Techo}{T_{2}^{\mathrm{echo}}}
\newcommand{\Gecho}{\Gamma_{\phi}^{\mathrm{echo}}}
\newcommand{\Gstar}{\Gamma_{\phi}^{\mathrm{*}}}
\newcommand{\Gphi}{\Gamma_\phi}
\newcommand{\Gqp}{\Gamma_\mathrm{qp}}
\newcommand{\xqp}{x_\mathrm{qp}}

% EJ EC
\newcommand{\EJ}{E_{\mathrm{J}}}
\newcommand{\EC}{E_{\mathrm{C}}}

\newcommand{\EJone}{E_{\mathrm{J1}}}
\newcommand{\EJtwo}{E_{\mathrm{J2}}}
\newcommand{\EJzero}{E_{\mathrm{J0}}}

% Sensitivity
\newcommand{\sens}{\left \vert\nicefrac{d\fzeroone}{d\Bperp}\right \vert}

\def\bra#1{\mathinner{\langle{#1}|}}
\def\ket#1{\mathinner{|{#1}\rangle}}
\def\braket#1{\mathinner{\langle{#1}\rangle}}
\def\Bra#1{\left\langle#1\right|}
\def\Ket#1{\left|#1\right\rangle}


\newcommand{\bran}{\langle n+1 \vert}

%frequencies
\newcommand{\fzeroone}{f_{01}}
\newcommand{\fzerotwoovertwo}{f_{02}/2}
\newcommand{\fonetwo}{f_{12}}
\newcommand{\fzerooneev}{f_{01}^{\mathrm{even}}}
\newcommand{\fzerooneodd}{f_{01}^{\mathrm{odd}}}
\newcommand{\fcav}{f_{\mathrm{c}}}


% Bperp Bpar1 Bpar2
\newcommand{\Bperp}{B_{\mathrm{\perp}}}
\newcommand{\Bparone}{B_{\mathrm{\parallel}, 1}}
\newcommand{\Bpartwo}{B_{\mathrm{\parallel}, 2}}
\newcommand{\Bpar}{B_{\mathrm{\parallel}}}

\newcommand{\Bx}{B_{\mathrm{x}}}
\newcommand{\By}{B_{\mathrm{y}}}
\newcommand{\Bz}{B_{\mathrm{z}}}

\newcommand{\Bcrit}{B^{\mathrm{crit}}}
\newcommand{\Bcritperp}{B_{\mathrm{\perp}}^{\mathrm{crit}}}
\newcommand{\Bcritparone}{B_{\mathrm{\parallel}, 1}^{\mathrm{crit}}}
\newcommand{\Bcritpar}{B_{\mathrm{\parallel}}^{\mathrm{crit}}}

\newcommand{\Bphinaught}{B_{\Phi_{0}}}
\newcommand{\Bphinaughtsquid}{B_{\Phi_{0},\mathrm{SQUID}}}

\newcommand{\sinc}{\mathrm{sinc}}

